Towards Jacamo-rest: A Resource-Oriented Abstraction for Managing Multi-Agent Systems

The Multi-Agent Oriented Programming (MAOP) paradigm provides abstractions to model and implements entities of agents, as well as of their organisations and environments. In recent years, researchers have started to explore the integration of MAOP and the resource-oriented web architecture (REST). This paper further advances this line of research by presenting an ongoing work on jacamo-rest, a resource-oriented web-based abstraction for the multi-agent programming platform JaCaMo. Jacamo-rest takes Multi-Agent System (MAS) interoperability to a new level, enabling MAS to not only interact with services or applications of the World Wide Web but also to be managed and updated in their specifications by other applications. To add a developer interface to JaCaMo that is suitable for the Web, we provide a novel conceptual perspective on the management of MAOP specification entities as web resources. We tested jacamo-rest using it as a middleware of a programming interface application that provides modern software engineering facilities such as continuous deployments and iterative software development for MAS.

==> Towards Jacamo-rest_ A Resource-Oriented Abstraction for Managing Multi-Agent Systems/old_notes.tex <==
\todo[inline]{This Section as a whole needs to be rewritten}

The main architectural style of the Web is resource-oriented, mostly in accordance with REST. It considers as a resource any information that can be named, for instance, an image, a document, a non-virtual object like a person and so on~\cite{fielding2000}. The architecture REST is not a technology itself and does not depends on a \textit{framework}. In contrast, REST is a specification, i.e., a model for developing web services.

REST refers to a style for transferring data in stateless textual representations~\cite{fielding2000}. In other words, REST considers each request as a unique operation which is independent of other requests that were performed before. REST specification for the Web uses standard requests of HTTP, the documents transfer protocol of the Web. Using just native requests makes REST compatible with other HTTP compliance services and applications, i.e., it is not necessary to add any abstraction layer to connect them. The data is transferred in text format. REST does not specify any text encoding of the payload; it can be HTML, XML, JSON or others.

REST services modelled using resource-oriented architecture (ROA), making proper use of HTTP verbs (GET, POST, PUT, DELETE and others), and allowing their Application Interfaces (APIs) be discovered by other systems are called RESTful~\cite{richardson2008restful}. This convention specifies more clearly how web services should be designed, making them easier to understand and interact with.

\todo{Rewrite}In REST, each accessible resource has a web address given by a Uniform Resource Identifier (URI). A URI may be used by different endpoints, for instance, to create, update or delete the referred resource. ``An endpoint is an abstraction that models the end of a message channel through which a system can send or receive messages''~\cite{Ibsen2010}. Through a URI, it is possible to specify parameters to retrieve specific data from an endpoint.


Hence, we introduce the following approach.
When a client requests an application state resource, it sends a \code{POST} request to create a \emph{snapshot} for the specified resource, for example to \code{/agents/\{agentuid\}/snapshots} (to get a snapshot of an agent's \emph{mind}).
The server then stores the current state of the resource and returns its UID to the client (\emph{e.g.}, \code{2b2cc71}).
Subsequently, the snapshot can be requested by any client at the corresponding UIR (\emph{e.g.}, \code{/agents/\{agentuid\}/snapshots/2b2cc71}).
Depending on how tightly resources are coupled, the server could also create snapshots of related application state objects and make them available under the same UID.

==> old_notes.tex <==
\todo[inline]{This Section as a whole needs to be rewritten}

The main architectural style of the Web is resource-oriented, mostly in accordance with REST. It considers as a resource any information that can be named, for instance, an image, a document, a non-virtual object like a person and so on~\cite{fielding2000}. The architecture REST is not a technology itself and does not depends on a \textit{framework}. In contrast, REST is a specification, i.e., a model for developing web services.

REST refers to a style for transferring data in stateless textual representations~\cite{fielding2000}. In other words, REST considers each request as a unique operation which is independent of other requests that were performed before. REST specification for the Web uses standard requests of HTTP, the documents transfer protocol of the Web. Using just native requests makes REST compatible with other HTTP compliance services and applications, i.e., it is not necessary to add any abstraction layer to connect them. The data is transferred in text format. REST does not specify any text encoding of the payload; it can be HTML, XML, JSON or others.

REST services modelled using resource-oriented architecture (ROA), making proper use of HTTP verbs (GET, POST, PUT, DELETE and others), and allowing their Application Interfaces (APIs) be discovered by other systems are called RESTful~\cite{richardson2008restful}. This convention specifies more clearly how web services should be designed, making them easier to understand and interact with.

\todo{Rewrite}In REST, each accessible resource has a web address given by a Uniform Resource Identifier (URI). A URI may be used by different endpoints, for instance, to create, update or delete the referred resource. ``An endpoint is an abstraction that models the end of a message channel through which a system can send or receive messages''~\cite{Ibsen2010}. Through a URI, it is possible to specify parameters to retrieve specific data from an endpoint.


Hence, we introduce the following approach.
When a client requests an application state resource, it sends a \code{POST} request to create a \emph{snapshot} for the specified resource, for example to \code{/agents/\{agentuid\}/snapshots} (to get a snapshot of an agent's \emph{mind}).
The server then stores the current state of the resource and returns its UID to the client (\emph{e.g.}, \code{2b2cc71}).
Subsequently, the snapshot can be requested by any client at the corresponding UIR (\emph{e.g.}, \code{/agents/\{agentuid\}/snapshots/2b2cc71}).
Depending on how tightly resources are coupled, the server could also create snapshots of related application state objects and make them available under the same UID.
